Investigation and improvements of the mechanical structure of Cylindrical GEMs for the BESIII experiment

Gas Electron Multipliers (GEMs) can be produced in large foils and molded in different shapes. The possibility to create cylindrical layers has opened the opportunity to use such detector as internal tracker at collider experiments. One crucial item is to have low material budget in the active area, so the supporting structure of anode and cathode must be light. KLOE2 collaboration has built the first Cylindrical GEM detector with honeycomb material with carbon fiber skins produced at high temperature. BESIII is developing an innovative CGEM detector with charge and time readout. Among several innovative features, the mechanical structure was designed to be a sandwich of Rohacell and Kapton, a PMI foam. After the transportation of a first production of the detectors from the construction site in Italy to the Institute of High Energy Physics in Beijing, some malfunctions have been observed in some of them, compatible with GEMs deformation inside the detector. We have performed a detailed study by means of an industrial CT scan available in IHEP laboratory and autopsy to the damaged detectors. In this talk, we will review the construction process, the shipment, the findings of the investigation. A new supporting structure of carbon fiber and honeycomb, assembled at room temperature, has been designed and developed. The thickness of the carbon fiber is small enough to keep the material budget of a single detector layer below 0.5$\%$ of a radiation length, while the mechanical robustness results beyond the purpose of a detector for HEP. A first detector with such a mechanical structure has been built and shipped to IHEP, preliminary results from operation (e.g. current stability, discharges, temperature and humidity correlation) of the detectors will be also presented in this talk.

==> pscompress <==
#!/bin/csh -f
while ($1 != "") 
	if (-e $1.bb || -e $1.Z) then
		echo will not overwrite $1.bb or $1.Z, skipping
		shift
	else 
		echo "%\!" > $1.bb
		grep \%\%BoundingBox $1 >> $1.bb
		compress $1
		shift
	endif
end

